On stability and stabilization of elastic systems by time-variant feedback

We study a class of elastic systems described by a (hyperbolic) partial differential equation. Our working example is the equation of a vibrating string subject to linear disturbance. The main goal is to establish conditions for stabilization and asymptotic stabilization by applying a fast oscillating control to the string. In the first situation studied we assume that system is subject to a damping force; next we consider the system without damping. We extend the tools of high-order averaging and of chronological calculus for studying stability of this distributed parameter system.

==> elastic_def.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{amsmath,amsfonts,amssymb}
%\usepackage{accents} %diversifica o tipo de acentos
\usepackage{graphicx}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage{calrsfs} %muda o estilo mathcal
\DeclareSymbolFont{rsfscript}{OMS}{rsfs}{m}{n}
\DeclareSymbolFontAlphabet{\mathrsfs}{rsfscript}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclareMathOperator{\z}{\mathbf{0}_2} \DeclareMathOperator{\Ad}{Ad}
\DeclareMathOperator{\ad}{ad} \DeclareMathOperator{\cD}{\mathrsfs{D}}
%\DeclareMathOperator{\cF}{\mathrsfs{F}}
\DeclareMathOperator{\cL}{\mathrsfs{L}} \DeclareMathOperator{\chro}{
\overleftarrow{\exp}} \DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\e}{e} \DeclareMathOperator{\id}{I}
\DeclareMathOperator{\l2}{L_2(\Omega)}
\DeclareMathOperator{\R}{\mathbb{R}}
\DeclareMathOperator{\sig}{\sigma} \DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\W}{\mathring{W}_2^1}
\DeclareMathOperator{\Wd}{\mathring{W}_2^2}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\numberwithin{equation}{section}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newtheorem{fct}{Assumption}
\newtheorem{thm}{Theorem}
%\newtheorem{lm}[thm]{Lemma}
\newtheorem{prp}{Proposition}
\newtheorem{dfn}{Definition}
\newtheorem{rmk}{Remark}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\lo}{L_2(\Omega)}
\newcommand{\veps}{\varepsilon}
\newcommand{\cF}{\mathrsfs{F}}
%\renewcommand{\thetheorem}{Theorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

